First Results from the $Herschel$ and ALMA Spectroscopic Surveys of the SMC: The Relationship Between [CII]-bright Gas and CO-bright Gas at Low Metallicity

The Small Magellanic Cloud (SMC) provides the only laboratory to study the structure of molecular gas at high resolution and low metallicity. We present results from the Herschel Spectroscopic Survey of the SMC (HS$^{3}$), which mapped the key far-IR cooling lines [CII], [OI], [NII], and [OIII] in five star-forming regions, and new ALMA 7m-array maps of $^{12}$CO and $^{13}$CO $(2-1)$ with coverage overlapping four of the five HS$^{3}$ regions. We detect [CII] and [OI] throughout all of the regions mapped. The data allow us to compare the structure of the molecular clouds and surrounding photodissociation regions using $^{13}$CO, CO, [CII], and [OI] emission at $<10$" ($<3$ pc) scales. We estimate Av using far-IR thermal continuum emission from dust and find the CO/[CII] ratios reach the Milky Way value at high A$_{V}$ in the centers of the clouds and fall to $\sim{1/5-1/10}\times$ the Milky Way value in the outskirts, indicating the presence of translucent molecular gas not traced by bright CO emission. We estimate the amount of molecular gas traced by bright [CII] emission at low A$_{V}$ and bright CO emission at high A$_{V}$. We find that most of the molecular gas is at low A$_{V}$ and traced by bright [CII] emission, but that faint CO emission appears to extend to where we estimate the H$_{2}$-to-HI transition occurs. By converting our H$_{2}$ gas estimates to a CO-to-H$_{2}$ conversion factor ($X_{CO}$), we show that $X_{CO}$ is primarily a function of A$_{V}$, consistent with simulations and models of low metallicity molecular clouds.

==> table1.tex <==
%% This is file `Table1.tex',
\ProvidesFile{table1.tex}
%
\begin{center}
\begin{deluxetable*}{@{\extracolsep{4pt}}lcccccc@{}}
\tablecolumns{7}
%\tablewidth{0pc}
\tablecaption{HS$^{3}$ \CII\ and \OI\ Map Properties \label{table:HS3}}
\tablehead{ & & & & & \multicolumn{2}{c}{$1\sigma$ Uncertainty} \\
 & \multicolumn{2}{c}{Center Position} &  &  & \multicolumn{2}{c}{($10^{-9}$ W m$^{-2}$ sr$^{-1}$)} \\
\cline{2-3} \cline{6-7}
\colhead{Region} & \colhead{R. A. (J2000)} & \colhead{Dec. (J2000)} & \colhead{Size} & \colhead{P. A.} & \colhead{\CII} & \colhead{\OI}} 
\startdata
 SWBarS & 00h45m27.10s & $-73$d21m00.00s & $1.7\arcmin \times 6.1\arcmin$ & 10\degr & 1.2 & 4.1 \\
 N22 & 00h47m58.10s & $-73$d16m52.13s & $1.7\arcmin \times 6.1\arcmin$ & 20\degr & 1.4 & 3.5 \\
 SWBarN & 00h48m26.88s & $-73$d06m04.36s  & $1.7\arcmin \times 6.1\arcmin$ & 145\degr & 1.5 & 3.9 \\
 SWDarkPK & 00h52m23.70s & $-73$d14m49.00s & $1.2\arcmin \times 1.2\arcmin$ & 48\degr & 1.3 & 3.4 \\
 N83 & 01h14m19.28s & $-73$d15m09.04s & $1.7\arcmin \times 8.0\arcmin$ & 30\degr & 1.4 & 3.5
\enddata
\end{deluxetable*}
\end{center}
\endinput

==> table2.tex <==
%% This is file `Tabl2w.tex',
\ProvidesFile{table2.tex}
%
\begin{center}
\begin{deluxetable*}{@{\extracolsep{4pt}}lccccccc@{}}
\tablecolumns{7}
%\tablewidth{0pc}
\tablecaption{HS$^{3}$ \NII\ and \OIII\ Map Properties \label{table:HS3_NII_OIII}}
\tablehead{ & & & & & & \multicolumn{2}{c}{$1\sigma$ Uncertainty} \\
 & \multicolumn{2}{c}{Center Position} &  & \multicolumn{2}{c}{P. A.} & \multicolumn{2}{c}{($10^{-9}$ W m$^{-2}$ sr$^{-1}$)} \\
\cline{2-3} \cline{5-6} \cline{7-8}
\colhead{Region} & \colhead{R. A. (J2000)} & \colhead{Dec. (J2000)} & \colhead{Size} & \colhead{\NII} & \colhead{\OIII} & \colhead{\NII} & \colhead{\OIII}} 
\startdata
 SWBarS & 00h45m21.85s & $-73$d22m49.36s & $1.5\arcmin \times 1.5\arcmin$ & 75\degr & 10\degr & 0.34 & 2.8 \\
 N22 & 00h47m54.35s & $-73$d17m27.69s & $1.5\arcmin \times 1.5\arcmin$ & 65\degr & 40\degr & 0.36 & 2.8 \\
 SWBarN & 00h48m26.30s & $-73$d06m04.28s  & $1.5\arcmin \times 1.5\arcmin$ & 75\degr & 55\degr & 0.27 & 2.4 \\
 SWDarkPK & 00h52m56.11s & $-73$d12m17.25s & $1\arcmin \times 1\arcmin$ & 55\degr & 40\degr & 0.33 & 2.8 \\
 N83 & 01h14m03.28s & $-73$d17m06.81s & $1.5\arcmin \times 1.5\arcmin$ & 50\degr & 65\degr & 0.29 & 3.0 
\enddata
\end{deluxetable*}
\end{center}
\endinput

==> table3.tex <==
%% This is file `Table3.tex',
\ProvidesFile{table3.tex}
%
\begin{center}
\begin{deluxetable*}{@{\extracolsep{4pt}}lcccc@{}}
\tablecolumns{5}
%\tablewidth{0pc}
\tablecaption{ALMA ACA+TP Map Properties \label{table:ALMA}}
\tablehead{ & \multicolumn{2}{c}{Map Center} & & \\
\cline{2-3} 
\colhead{Region} & \colhead{R. A. (J2000)} & \colhead{Dec. (J2000)} & \colhead{Map Size} & \colhead{P. A.}} 
\startdata
 SWBarS & 00h45m24.54s & $-73$d21m42.63s & $2.3\arcmin \times 3.5\arcmin$ & 10\degr \\
 N22 & 00h47m54.28s & $-73$d17m46.76s & $2.3\arcmin \times 3.5\arcmin$ & 20\degr \\
 SWBarN & 00h48m15.53s & $-73$d04m56.41s & 2.3$\arcmin\times 3.5\arcmin$ & 145\degr \\
 SWDarkPK & 00h52m56.07s & $-73$d12m17.08s & $3\arcmin \times 3\arcmin$ & 48\degr 
\enddata

\end{deluxetable*}
\end{center}
\endinput

==> table3b.tex <==
%% This is file `Table3.tex',
\ProvidesFile{table3b.tex}
%
\begin{center}
\begin{deluxetable*}{@{\extracolsep{4pt}}lcccccc@{}}
\tablecolumns{7}
%\tablewidth{0pc}
\tablecaption{ALMA ACA+TP Map Properties (continued) \label{table:ALMA_cont}}
\tablehead{ & \multicolumn{3}{c}{ $\theta_{maj}(\arcsec)\times\theta_{min}(\arcsec)$} & \multicolumn{3}{c}{RMS (K)} \\
\cline{2-4} \cline{5-7} 
\colhead{Region} &\colhead{\CO} & \colhead{\thirteenCO} & \colhead{\CeighteenO} & \colhead{\CO} & \colhead{\thirteenCO} & \colhead{\CeighteenO} } 
\startdata
 SWBarS & $6.60\times6.06$ & $6.92\times6.05$ & $6.76\times6.18$ & 0.17 & 0.16 & 0.10 \\
 N22 & $6.39\times5.56$ & $6.59\times5.83$ & $7.01\times6.41$ & 0.24 & 0.22 & 0.13  \\
 SWBarN & $7.08\times5.74$ & $7.25\times5.33$ & $7.40\times5.66$ & 0.12 & 0.16 & 0.08 \\
 SWDarkPK & $6.95\times5.55$ & $8.39\times5.63$ & $7.42\times5.72$ & 0.18 & 0.16 & 0.10 
\enddata
\end{deluxetable*}
\end{center}
\endinput

==> table4.tex <==
%% This is file `Table4.tex',
\ProvidesFile{table4.tex}
%
\begin{deluxetable*}{@{\extracolsep{4pt}}lcccccc@{}}
\tablecolumns{7}
%\tablewidth{0pc}
\tablecaption{ALMA CO Properties \label{table:ALMA_prop}}
\tablehead{ & & \multicolumn{2}{c}{$T_{peak}$\tablenotemark{a} (K)} & \multicolumn{3}{c}{Map Sensitivity\tablenotemark{b} (K km s$^{-1}$)}\\
\cline{3-4} \cline{5-7}
\colhead{Region} & \colhead{$\Delta{v_{\rm{LSR}}}$ (km s$^{-1}$)} & \colhead{\CO} & \colhead{\thirteenCO} & \colhead{\CO} & \colhead{\thirteenCO} & \colhead{\CeighteenO} }  
\startdata
 SWBarS & $104-133$ & 18.6 & 4.9 & 2.1 & 1.7 & 1.2 \\
 N22 & $113-133$ & 15.9 & 2.6 & 2.1 & 2.4 & 1.0 \\
 SWBarN & $104-140$ & 14.6 & 4.3 & 1.8 & 2.2 & 1.2 \\
 SWDarkPK & $137-160$ & 12.1 & 3.0 & 1.9 & 1.8 & 1.3
\enddata
\tablenotetext{a}{in 0.3 km s$^{-1}$ channels}
\tablenotetext{b}{defined as $3\times{RMS}$ in regions away from line emission}
\end{deluxetable*}
\endinput

==> table5.tex <==
%% This is file `Table5.tex',
\ProvidesFile{table5.tex}
%
\begin{center}
\begin{deluxetable*}{@{\extracolsep{4pt}}lccccccc@{}}
\tablecolumns{8}
\tablewidth{0pc}
\tablecaption{Properties of \htwo\ Estimates from \CII\ \label{table:h2_estimates}}
\tablehead{ & \multicolumn{2}{c}{Average \% $I_{\CII}$} & \multicolumn{2}{c}{$\bar{N}_{\htwo,\CII}$ [$10^{21}$ cm$^{-2}$]} & \multicolumn{2}{c}{$M_{\htwo,\CII}$ [$10^{4}$ \msol]} &  \\
\cline{2-3} \cline{4-5} \cline{6-7} 
\colhead{Region} & \colhead{from \hi} & \colhead{from H$^{+}$} & \colhead{Fixed $T,~n$} & \colhead{W16} & \colhead{Fixed $T,~n$} & \colhead{W16} & \colhead{$M_{\htwo,\CO}$ [$10^{4}$ \msol]}} 
\startdata
 SWBarS & 3\% & 6\% & 1.2 & 0.97 & 5.05 & 4.15 & 1.3 \\
 N22 &  2\% & 15\% & 1.6 & 1.1 & 5.64 & 4.13 & 1.0 \\
 SWBarN & 2\% & 7\% & 2.9 & 2.5 & 8.60 & 7.21 & 1.7 \\
 SWDarkPK & 7\% & 9\% & 0.48 & 0.63 & 0.90 & 1.16 & 0.10
\enddata
\end{deluxetable*}
\end{center}
\endinput

==> table5a.tex <==
%% This is file `Table5a.tex',
\ProvidesFile{table5a.tex}
%
\begin{center}
\begin{deluxetable}{@{\extracolsep{4pt}}lccccccc@{}}
\tablecolumns{8}
\tablewidth{0pc}
\tablecaption{\htwo\ Estimate from \CII\ Uncertainties \label{table:h2_estimates_unc}}
\tablehead{ \colhead{Source of Uncertainty} & \colhead{Uncertainty Estimate}} 
\startdata
PACS Calibration & $\pm30\%$ \\
Carbon Abundance & $\pm30\%$ \\
\OI\ Absorption & $-30\%$ \\
\CII\ Optical Depth & $+10\%$ \\
PDR Model Metallicity & factor of 2
\enddata
\end{deluxetable}
\end{center}
\endinput

==> table6.tex <==
%% This is file `Table6.tex',
\ProvidesFile{table6.tex}
%
\begin{center}
\begin{deluxetable}{@{\extracolsep{4pt}}lcccc@{}}
\tablecolumns{5}
\tablewidth{0pc}
\tablecaption{Total Gas Masses \label{table:gas_masses}}
\tablehead{ & \multicolumn{2}{c}{$M_{\htwo}$ [$10^{5}$ \msol]} & \multicolumn{2}{c}{$M_{\hi}$ [$10^{5}$ \msol]} \\ 
\cline{2-3} \cline{4-5}
\colhead{Region} & \colhead{\CII+CO} & \colhead{Dust} & \colhead{$\Delta{v}_{\rm{CO}}$\tablenotemark{a}} & \colhead{$\Delta{v}_{\rm{total}}$} }
\startdata
 SWBarS & $0.52^{+0.52}_{-0.26}$ & $2.33^{+2.33}_{-1.17}$ & 3.42 & 6.53 \\
 N22 & $0.48^{+0.48}_{-0.24}$ & $1.23^{+1.23}_{-0.62}$ & 3.15 & 7.30 \\
 SWBarN & $0.86^{+0.86}_{-0.43}$ & $1.61^{+1.61}_{-0.81}$ & 4.64 & 9.00 \\
 SWDarkPK & $0.11^{+0.11}_{-0.06}$ & $1.79^{+1.79}_{-0.90}$ & 1.46 & 3.08 \\
 N83 & $0.48^{+0.48}_{-0.24}$ & $2.96^{+2.96}_{-1.48}$ & 4.67 & 6.16 
\enddata
\tablenotetext{a}{using the \hi\ integrated intensity only around the velocity channels with CO emission}
\end{deluxetable}
\end{center}
\endinput
